Devito: Towards a generic Finite Difference DSL using Symbolic Python

Domain specific languages (DSL) have been used in a variety of fields to express complex scientific problems in a concise manner and provide automated performance optimization for a range of computational architectures. As such DSLs provide a powerful mechanism to speed up scientific Python computation that goes beyond traditional vectorization and pre-compilation approaches, while allowing domain scientists to build applications within the comforts of the Python software ecosystem. In this paper we present Devito, a new finite difference DSL that provides optimized stencil computation from high-level problem specifications based on symbolic Python expressions. We demonstrate Devito's symbolic API and performance advantages over traditional Python acceleration methods before highlighting its use in the scientific context of seismic inversion problems.

==> makefile <==
TARGET   = devito-pyhpc
PDFLATEX = pdflatex
DOCS     = devito-pyhpc.tex preamble.tex abstract.tex \
	intro.tex background.tex devito_design.tex example_diffusion.tex \
	example_acoustic.tex discussion.tex figures/devito_layers.tex
BIBINPUTS = references.bib


devito-pyhpc.pdf: devito-pyhpc.tex ${DOCS} ${BIBINPUTS}
	rm -f devito-pyhpc.bbl
	${PDFLATEX} $<
	bibtex ${TARGET}
	${PDFLATEX} $<
	${PDFLATEX} $<

clean:
	rm -f ${TARGET}.out ${TARGET}.aux ${TARGET}.bbl ${TARGET}.blg ${TARGET}.log ${TARGET}.pdf

simple:	${TARGET}.pdf

default: devito-pyhpc.pdf

.PHONY: simple

